3PSDF: Three-Pole Signed Distance Function for Learning Surfaces with Arbitrary Topologies

Recent advances in learning 3D shapes using neural implicit functions have achieved impressive results by breaking the previous barrier of resolution and diversity for varying topologies. However, most of such approaches are limited to closed surfaces as they require the space to be divided into inside and outside. More recent works based on unsigned distance function have been proposed to handle complex geometry containing both the open and closed surfaces. Nonetheless, as their direct outputs are point clouds, robustly obtaining high-quality meshing results from discrete points remains an open question. We present a novel learnable implicit representation, called the three-pole signed distance function (3PSDF), that can represent non-watertight 3D shapes with arbitrary topologies while supporting easy field-to-mesh conversion using the classic Marching Cubes algorithm. The key to our method is the introduction of a new sign, the NULL sign, in addition to the conventional in and out labels. The existence of the null sign could stop the formation of a closed isosurface derived from the bisector of the in/out regions. Further, we propose a dedicated learning framework to effectively learn 3PSDF without worrying about the vanishing gradient due to the null labels. Experimental results show that our approach outperforms the previous state-of-the-art methods in a wide range of benchmarks both quantitatively and qualitatively.

==> figures/fig_rebut_binary.tex <==
\begin{figure}[!htb]
    \centering
    \vspace{-3mm}
    \begin{overpic}[width=\linewidth]{figs/pl/fig_rebut_binary.png}
    \put(1, -5) {\footnotesize input}
    \put(21,-5) {\footnotesize ours-occ}
    \put(52, -5){\footnotesize ours-3psdf}
    \put(90, -5){\footnotesize GT}
    
    \put(115, -5) {\footnotesize input}
    \put(140,-5) {\footnotesize ours-occ}
    \put(175, -5){\footnotesize ours-3psdf}
    \put(220, -5){\footnotesize GT}

    \end{overpic}
\caption{Implementation of OccNet using our network architecture. Ours-3PSDF: 1.27(CD), 0.75(F-Score); Ours-Occ: 2.06(CD), 0.68(F-Score).}
\label{fig:rebut_binary}
\vspace{-3mm}
\end{figure}

==> figures/fig_rebut_geo_op.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{figs/raster/ndf_figure9.png}
\vspace{-5mm}
\caption{Geometry operations of 3PSDF.}
\label{fig:rebut_geo_op}
\end{figure}


==> package.tex <==













==> sections/exp_timing.tex <==
\subsection{Timing Cost for Field-to-Mesh Conversion}
\label{sec:exp_timing}

%\brandon{Sec 4.2 already discuss the performance superiority. Thus, this section only discuss the time here? Do we need separate them into two sections? We may need to describe the experiment settings again, leading to possible waste of paper space.}

%\weikai{Yes, we want to emphasize our time cost is extremely low compared to NDF -- that's why we use another subsection. We will use the same setting with Section~\ref{sec:exp_shape_recon}. So after explaining the setting in Section~\ref{sec:exp_shape_recon}, we can just say we use the same setting here. If it is a waste of space, we could end up merging them into one table and one subsection.}

\note{
\begin{itemize}
    \item Goal: We want to show our method can achieve much faster field-to-mesh conversion compared to the approaches based on unsigned distance field, e.g. NDF.
    \item Setting: Given a field representation of an open surface, compute the time of converting it into corresponding mesh.
    \item Dataset: 3D-Front + Mixamo + MGN
    \item Baselines: NDF 
\end{itemize}
}

==> tables/tab_MGN_scene.tex <==
\begin{table}[!htb]
  \centering
    \begin{tabular}{l||r||r}
    \hline
          & \multicolumn{2}{c}{Chamfer-$L_2$} \\
    \hline
          & \multicolumn{1}{c||}{MGN} & \multicolumn{1}{c}{3D-Front} \\
    \hline
    \hline
    NDF     & 0.035         & 1.452 \\
    Ours    &\textbf{0.033} &  \textbf{1.378} \\
    \midrule
    \end{tabular}
  \caption{Results of point cloud completion for MGN and 3D-Front from 3000 and 50000 points. Chamfer-$L_2$ distance is reported in $\times 10^{-4}$.}
  \label{tab:mgn_scene}
\end{table}%

==> tables/tab_point_car_closed.tex <==
\begin{table}[!htb]
  \centering
    \begin{tabular}{l||r||r}
    \hline
          & \multicolumn{2}{c}{Chamfer-$L_2$} \\
    \hline
          & \multicolumn{1}{c||}{3000 Points} & \multicolumn{1}{c}{300 Points} \\
    \hline
    \hline
    DMC     & 1.255         &  2.417 \\
    OccNet  & 0.938         & 1.009 \\
    IF-Net  & 0.326         &  1.147\\
    NDF     & 0.127         & 0.626 \\
    Ours    &\textbf{0.112} &  \textbf{0.595} \\
    \midrule
    \end{tabular}%
  \caption{Results of point cloud completion for closed watertight cars from 3000 and 300 points. Chamfer-$L_2$ distance is reported in $\times 10^{-4}$.}
    \label{tab:car_close_cd}%
\end{table}%

==> tables/tab_point_car_open.tex <==
\begin{table}[!htb]
  \centering
    \begin{tabular}{l||r||r}
    \hline
          & \multicolumn{2}{c}{Chamfer-$L_2$} \\
    \hline
          & \multicolumn{1}{c||}{10000 Points} & \multicolumn{1}{c}{3000 Points} \\
    \hline
    \hline
    SAL  & 6.39             & 7.39 \\
    NDF  & 0.074            & 0.275 \\
    Ours & \textbf{0.071}   & \textbf{0.258} \\
    \midrule
    \end{tabular}
  \caption{Results of point cloud completion for unprocessed cars from 10000 and 3000 points. Chamfer-$L_2$ distance is reported in $\times 10^{-4}$.}
    \label{tab:car_open_cd}%
\end{table}%



==> tables/tab_rebut_fscore.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c||c||c|c|c|c|c}
    \hline
     & \multirow{2}{*}{Method} & \multicolumn{5}{c}{ShapeNet}  \\
     \cline{3-7} & & car & plane & boat & lamp & chair  \\
    % \midrule
    \hline
    \hline
    \multirow{3}{*}{FS  $\uparrow$} 
    & IMNet   & 31.8  & 33.7 & 39.8 & 34.3  & 61.1  \\
     & OccNet    &54.4  & 59.7  & 44.9  &  \textbf{50.6} & 59.6  \\
     & DISN    & 65.8  & \textbf{77.2}  & 57.8 & 50.4 & \textbf{63.8}   \\
    %  & NDF    &  &  &   &  &   \\
     & Ours & \textbf{77.0} & 72.8 & \textbf{66.6} & 49.3 & 58.5  \\
    \midrule
\end{tabular}
\end{center}
\vspace{-5mm}
\caption{F-score evaluation.}
\label{tab:rebut_fscore}
\vspace{-3mm}
\end{table}

==> tables/tab_rebut_median.tex <==
\begin{table}[!htb]
\vspace{-3mm}
	\begin{minipage}[t]{.5\linewidth}
		\centering
		\begin{tabular}[t]{l||r||r}
			\hline
			& \multicolumn{2}{c}{Chamfer-$L_2$} \\
			\hline
			& \multicolumn{1}{c||}{3K} & \multicolumn{1}{c}{300} \\
			\hline
			\hline
			DMC     & 0.560         &  0.973 \\
			OccNet  & 0.482         & 0.590 \\
			IF-Net  & 0.127         &  0.482\\
			NDF     & 0.055         & 0.371 \\
			Ours    &\textbf{0.049} &  \textbf{0.356} \\
			\midrule
		\end{tabular}%		
	\end{minipage}%
	\begin{minipage}[t]{.5\linewidth}
		\centering
		\begin{tabular}[t]{l||r||r}
			\hline
			& \multicolumn{2}{c}{Chamfer-$L_2$} \\
			\hline
			& \multicolumn{1}{c||}{10K} & \multicolumn{1}{c}{3K} \\
			\hline
			\hline
			SAL  & 5.79             & 5.44 \\
			NDF  & 0.041            & \textbf{0.086} \\
			Ours & \textbf{0.039}   & {0.087} \\
			\midrule
		\end{tabular}%
	\end{minipage} 
	\vspace{-3mm}
% \caption{Median value of Table 2 of the main paper.}
\label{tab:rebut_median}
\end{table}

==> tables/tab_rebut_regress.tex <==
\begin{table}[h]
\begin{center}
\begin{tabular}{c||c||c|c|c|c|c}
    \hline
     & \multirow{2}{*}{Method} & \multicolumn{5}{c}{ShapeNet}  \\
     \cline{3-7} & & car & plane & boat & lamp & chair  \\
    % \midrule
    \hline
    \hline
    \multirow{3}{*}{FS  $\uparrow$} 
    & IMNet   & 31.8  & 33.7 & 39.8 & 34.3  & 61.1  \\
     & OccNet    &54.4  & 59.7  & 44.9  &  \textbf{50.6} & 59.6  \\
     & DISN    & 65.8  & \textbf{77.2}  & 57.8 & 50.4 & \textbf{63.8}   \\
    %  & NDF    &  &  &   &  &   \\
     & Ours & \textbf{77.0} & 72.8 & \textbf{66.6} & 49.3 & 58.5  \\
    \midrule
\end{tabular}
\end{center}
\vspace{-5mm}
\caption{Quantitative evaluation of different learning methods of 3PSDF.}
\label{tab:rebut_regress}
\vspace{-3mm}
\end{table}
